Making Distributed Mobile Applications SAFE: Enforcing User Privacy Policies on Untrusted Applications with Secure Application Flow Enforcement

Today's mobile devices sense, collect, and store huge amounts of personal information, which users share with family and friends through a wide range of applications. Once users give applications access to their data, they must implicitly trust that the apps correctly maintain data privacy. As we know from both experience and all-too-frequent press articles, that trust is often misplaced. While users do not trust applications, they do trust their mobile devices and operating systems. Unfortunately, sharing applications are not limited to mobile clients but must also run on cloud services to share data between users. In this paper, we leverage the trust that users have in their mobile OSes to vet cloud services. To do so, we define a new Secure Application Flow Enforcement (SAFE) framework, which requires cloud services to attest to a system stack that will enforce policies provided by the mobile OS for user data. We implement a mobile OS that enforces SAFE policies on unmodified mobile apps and two systems for enforcing policies on untrusted cloud services. Using these prototypes, we demonstrate that it is possible to enforce existing user privacy policies on unmodified applications.

==> Makefile <==
# Use bash for expansions
SHELL=/bin/bash
null=
space= $(null) #
comma= ,

LATEX=latexmk -synctex=1 -bibtex -f- -pdf -interaction=nonstopmode -halt-on-error
LATEXRUN=./bin/latexrun --color auto -W no-overfull -W no-citation --latex-args '\-synctex=1'
PAPER=paper

# ASPELL_CMDS SYNTAX: command_name argstring
#                         'p'/'P' in argstring indicates mandatory parameter
#                         'o'/'O' in argstring indicates optional parameter
#                         ignores parameter, uppercase doesn't
ASPELL_CMDS=\
	--add-tex-command='addfig p' \
	--add-tex-command='addgraph p' \
	--add-tex-command='autoref p' \
	--add-tex-command='begin pop' \
	--add-tex-command='bibliography p' \
	--add-tex-command='bibliographystyle p' \
	--add-tex-command='citeauthor p' \
	--add-tex-command='color p' \
	--add-tex-command='cref p' \
	--add-tex-command='Crefname ppp' \
	--add-tex-command='DeclareMathOperator pp' \
	--add-tex-command='definecolor ppp' \
	--add-tex-command='eqref p' \
	--add-tex-command='fvset p' \
	--add-tex-command='hypersetup p' \
	--add-tex-command='lstinputlisting o' \
	--add-tex-command='lstset p' \
	--add-tex-command='mathit p' \
	--add-tex-command='mathrm p' \
	--add-tex-command='mathtt p' \
	--add-tex-command='newcommand pp' \
	--add-tex-command='PassOptionsToPackage pp' \
	--add-tex-command='providecommand pp' \
	--add-tex-command='renewcommand pp' \
	--add-tex-command='special p' \
	--add-tex-command='texttt p' \
	--add-tex-command='usetikzlibrary p' \
	--add-tex-command='VerbatimInput p' \

TEX=$(filter-out ./flat.tex, $(shell find ./ -type f -name "*.tex"))
CLS=$(shell find ./ -type f -name "*.cls" -or -name "*.sty")
BIB=$(shell find ./ -type f -name "*.bib")

# Should list all source files to paper (i.e., all files manually edited)
SRC=$(TEX) $(CLS) $(BIB)

.PHONY: all clean viewpdf continuous-update latexrun continuous-update-lr spell \
				checkturnin
.FORCE:

all: $(PAPER).pdf

$(PAPER).pdf: $(SRC)
	@ rm -fv .option-overrides.tex
	@ echo "[latexmk] $@"
	@ # Only compile with verbose if the quiet build fails
	@ $(LATEX) $(PAPER).tex -quiet || $(LATEX) $(PAPER).tex
	@ # Comment because latexmk annoyingly doesn't end output with a newline

latexrun: $(SRC)
	@ rm -fv .option-overrides.tex
	@ echo "[latexrun] $(PAPER).pdf"
	@ $(LATEXRUN) -O .latex.out $(PAPER).tex
	@ cp .latex.out/$(PAPER).synctex.gz ./

$(PAPER)-TR.pdf: $(SRC)
	@ echo '\trtrue' > .option-overrides.tex
	@ echo "[latexrun] $@"
	@ $(LATEXRUN) $(PAPER).tex -O .latex.out.TR -o $@
	@ cp .latex.out.TR/$(PAPER).synctex.gz ./$(PAPER)-TR.synctex.gz
	@ rm -fv .option-overrides.tex

continuous-update:
	@ watchy -i '^$$' -w $(subst $(space),$(comma),$(SRC)) make

continuous-update-lr:
	@ watchy -i '^$$' -w $(subst $(space),$(comma),$(SRC)) make latexrun $(PAPER)-TR.pdf

viewpdf: $(PAPER).pdf
	gnome-open $(PAPER).pdf

diff-%.pdf: .FORCE
	./bin/git-latexdiff --main $(PAPER).tex $* -- \
		--exclude-textcmd="section,subsection,subsubsection,dontdifthis" -o $@

flat.tex: $(TEX) $(CLS)
	./bin/latexpand --expand-usepackage --empty-comments --verbose -o $@ $(PAPER).tex
	perl -i -p0e 's/\\iftr(?:(?!\\(?:fi|else|iftr)).)*\\else((?:(?!\\(?:fi|else|iftr)).)*)\\fi/$$1/seg' $@ # replace \iftr \else \fi
	perl -i -p0e 's/\\iftr(?:(?!\\(?:fi|else|iftr)).)*\\fi//seg' $@ # replace \iftr \fi
	sed -i 's/\s*$$//' $@ # strip trailing spaces
	sed -i '/^\s*\%$$/d' $@ # strip comment-only lines
	sed -i 'N;/^\n$$/D;P;D;' $@ # replace multiple empty newlines with one
	perl -i -0pe 's/^.*(?=\\documentclass)//s' $@ # trim everything before documentclass

turnin.zip: flat.tex $(PAPER).pdf $(BIB) \
						$(shell find ./figures -type f -not -path "*.graffle*")
	zip $@ $^

checkturnin: turnin.zip $(PAPER).pdf .FORCE
	rm -rf /tmp/turnin-check-n10dfl
	mkdir /tmp/turnin-check-n10dfl
	cp $< lipics-v2016.cls lipics-logo-bw.pdf cc-by.pdf /tmp/turnin-check-n10dfl
	cd /tmp/turnin-check-n10dfl; unzip $<; $(LATEX) flat.tex -quiet -f
	diffpdf $(PAPER).pdf /tmp/turnin-check-n10dfl/flat.pdf
	rm -rf /tmp/turnin-check-n10dfl

spell: $(SPELL_SCRIPTS)
	@ echo "------ Spellchecking ------"
	@ echo "(Does not check bibliography.)"
	@ for i in $(TEX);\
			do aspell --lang=en_US -t $(ASPELL_CMDS) -p ./.aspell.words -c $$i;\
		done
	@ echo -e "\n------ Double words ------"
	@ for i in $(TEX);\
			do bin/double.pl $$i;\
		done
	@ echo -e "\n------ Abbreviations at end of sentences ------"
	@ for i in $(TEX);\
			do bin/abbrv.pl  $$i;\
		done
	@ echo -e "\n------ Passive voice ------"
	@ bash bin/passive.sh $(TEX)
	@ echo -e "\n------ Hyphenated ly words ------"
	@ bash bin/hyphens.sh $(TEX)
	@ echo -e "\n------ Weasel words ------"
	@ bash bin/weasel.sh $(TEX)
	@ # Sort the added words
	@ (head -1 .aspell.words ; tail -n +2 .aspell.words | LC_ALL=C sort) \
		> .aspell.words~
	@ mv .aspell.words~ .aspell.words

summary: summary.pdf

summary.pdf: summary.tex
	@ rm -fv .option-overrides.tex
	@ echo "[latexmk] $@"
	@ # Only compile with verbose if the quiet build fails
	@ $(LATEX) summary.tex -quiet || $(LATEX) summary.tex
	@ # Comment because latexmk annoyingly doesn't end output with a newline

clean:
	@ latexmk -c > /dev/null 2>&1
	@ rm -frv latex.out .latex.out .latex.out.TR $(PAPER).synctex.gz .option-overrides.tex
	@ rm -fv $(PAPER){,-TR}.{dvi,ps,gz,log,blg,image.tex,brf,haux,htoc,hbbl,out,tdo,pdf,synctex.gz,vtc} pdflatex*.fls
	@ rm -fv summary.{dvi,ps,gz,log,bbl,blg,image.tex,brf,haux,htoc,hbbl,out,tdo,pdf,synctex.gz,vtc}
	@ find ./ -name "*.tex.bak" -delete
	@ rm -fv diff-*.pdf
	@ rm -fv flat.*
	@ rm -fv turnin.zip


==> arch.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-

This section defines


\subsection{System Model}

Figure~\ref{fig:arch} shows the \agate architecture.  An {\em \agate
  application} consists of a set of processes distributed across
mobile devices and back-end cloud servers.  Each Agate deployment
supports a single Agate application.  An Agate deployment consists of
several components: \squishlist
\item The \emph{\agate mobile OS} runs on each user's mobile
  device. The OS manages user policies and provides a secure UI for
  users to set their sharing policies. It also interposes on any
  application access to an OS-protected resource to automatically
  label data from the resource.
\item The \emph{\agate distributed runtime platform} executes
  application code on cloud servers and uses fine-grained information
  flow control to track the flow of labeled data through untrusted
  application processes and enforce user policies. %  To implement
  % fine-grained IFC, the Agate runtime requires a managed language
  % environment (e.g., Java, Python, Scala, Ruby) -- a common choice for
  % cloud applications today.
\item A \emph{user management service} (UMS) -- similar to existing
  services like Google Accounts~\cite{googl_accoun} and Apple
  ID~\cite{apple_id} -- provides secure global user identities and
  group membership for expressing Agate policies and labels.  The UMS
  verifies the identity of each mobile device user, so Agate can label
  data from that device and control what data can flow to that
  device.  % The UMS is not an Agate-specific
  % component; \agate could integrate any existing service or
  % application that can verify user identities (e.g., Google
  % Accounts~\cite{googl_accoun}, Apple ID~\cite{apple_id}, Microsoft
  % Account~\cite{micros_accoun}) and support group membership (e.g.,
  % Google Circles).
\item An \emph{app store}, like the Apple App
  Store~\cite{apple_app_store} and Google Play
  Store~\cite{googl_play}, acts as a trusted distributor and
  identifier of Agate applications.  We trust the app store to
  securely implement Agate's implicit flow control mechanism by
  performing binary translation of the application bytecode (e.g., the
  Android apk) when users download and install Agate apps on their
  devices.  % However, this decision is an optimization to reduce
  % performance overhead at runtime, as the Agate runtime could also
  % perform the same translation.
\squishend

These components do not have to be deployed by a single provider;
however, each service provider must be trusted and they must have a
way to securely authenticate and communicate with each other.  For
example, the mobile OS may be provided by Google, while the
distributed runtime platform is provided by Facebook and user
authentication is provided by yet another party (e.g.,
OpenID~\cite{openid}).  In Section~\ref{sec:agate-platform}, we
discuss the requirements for authentication and verification to enable
the mobile OS to label data with authenticated user ids and pass that
labeled data to the distributed runtime platform.

\subsection{\agate Sharing Policies}
\label{sec:policies}
To minimize changes to the user experience, Agate policies match
existing user privacy policies as closely as possible.  To that end,
Agate integrates both types of privacy policies that users set today
into a single policy. \emph{Agate sharing policies} specify: (1) which
OS-protected resources an application can access, and (2) how the
application can export data derived from that resource.  For example,
in Figure~\ref{fig:arch}, \agate permits Alice's photo to be passed to
an application and then to Betty, while it prevents the photo from
being shared with Bob.  Note that Agate uses these policies for users
to express their privacy preferences \emph{and} for the IFC mechanism
to enforce those preferences.

\agate sharing policies are expressed in terms of \emph{users},
\emph{groups}, and \emph{applications}. Each policy maps an
OS-protected resource to an application that is allowed to access it
and the list of users and groups with which the app can share that
data.  For example, Alice can set a policy allowing her fitness app to
access her GPS and to share her GPS-derived data only with Betty. We
use the following notation to denote Alice's sharing policy:
$\resource{GPS} = \tup<\app{FitApp},\set{\principal{Betty}}>$. Note
that this policy only allows Fitapp to share Alice's GPS-derived data
with Betty, not other applications.  Users can also define policies
for their restricted resources. For example, to let another app share
Alice's current neighborhood but not her precise location with Betty,
Alice could define
$\exception{GPS}{Neighborhood} =
\tup<\app{FriendApp},\set{\principal{Betty}}>$.

% \agate's policies preserve the existing user experience. Users already
% have such policies in mind but typically specify them through
% in-application interfaces (e.g., a dialog box in which the user
% selects with whom to share a photo).  In contrast, \agate bypasses the
% application, securely collects user policies through its mobile OS and
% enforces those policies in the platform itself.

To minimize application changes, \agate allows applications to suggest
policies similar to the ones that apps provide and enforce today.
Apps create \agate groups that map to application-specific
concepts. For example, Alice's fitness application could define
$\group{Alice}{Running-Group}$, which lets Alice share her runs with
her running partners. \agate also provides an API for applications to
propose policies. For example, Alice's fitness app might offer her the
choices
%$\resource{GPS} = \tup<\app{FitApp}, \set{}>$
$\resource{GPS} = \tup<\app{FitApp}, \set{\principal{Alice}}>$ and
$\resource{GPS} = \tup<\app{FitApp}, \set{\principal{Alice},
  \group{Alice}{running-group}}>$
to only share data from the GPS across Alice's devices or with her
group.



% While Agate provides these four components, applications can choose to
% deploy a subset and replace an Agate component with a trusted
% component of some other kind.  However, in each case, the user must
% trust that the component that the application has chosen will
% correctly enforce their policies.  For example, an app could easily
% replace the UMS with another trusted identity service (e.g.,
% OpenID~\cite{openid}).  This change would not significantly impact An app could also replace the Agate runtime
% for back-end app processes in the cloud with another fine-grained IFC
% tracking system (e.g., Hails~\cite{giffin:hails}).
% Section~\ref{sec:agate-platform} specifies the requirements for each
% Agate component and how Agate components interact with other trusted
% components.



% Users log in to \agate through the secure UI, which identifies and
% authenticates users using the UMS.  Because most devices are designed
% to have a single user, \agate directly associates data and processes
% on a device with the logged-in user.
%   % Thus, mobile OS user id accomplishes three tasks: (1) it
% % associates a device with the user, (2) it allows \agate to enforce
% % policies on behalf of the user, and (3) it allows the user to run
% % \agate applications.
% Likewise, application processes on mobile devices or the cloud must
% identify themselves to the distributed runtime system when they begin
% executing to access OS-protected resources and receive data from other
% application processes.



\subsection{Trust and Threat Model}
While Agate strives to minimize changes for users and programmers, its
end goal is to reduce the trust that users must place on programmers
to enforce their privacy preferences.  To that end, we assume that
both the user and the applications trust \agate, but the user and
\agate have limited trust in applications.

%% Figure out wha the TPM story is
% We assume that users trust
% their devices to run the \agate mobile OS and their cloud provider to
% run the \agate distributed runtime (or other trusted components as we
% discuss in Section0. % These assumptions are reasonable because mobile
% devices are generally under the control of a single user, and the
% cloud provider is generally a trusted third party.  Alternatively,
% users could rely on trusted hardware components (e.g., TPM-based
% attestation) to ensure that untrusted cloud servers run the correct
% Agate software stack~\cite{ gasser89:_digit_distr_system_secur_archit,
%   arbaugh97:_secur_and_reliab_boots_archit,
%   sailer04:_desig_implem_tcg_integ_measur_archit,baumann14:haven}.

The trusted computing base for \agate includes everything in the stack
{\em below} the application on both mobile devices and cloud servers.
This includes all Agate components -- the mobile OS, the distributed
runtime platform, the user management service and the app store -- as
well as the cloud server software stack, including the OS and hypervisor.

While we trust all server hardware, we assume that users only trust
their own mobile devices. Thus, when a user adds a mobile device to
the \agate system, we assume that: (1) the device belongs to the user,
and (2) the user trusts the device to hold her data. We also assume
that when users give other users access to their data, they trust the
devices of those other users.  For example, if Alice gives Betty
access to her GPS location, Alice must trust any device that Betty is
willing to log into.

\paragraph{Timing, termination and probabilistic channels.} \agate's
ability to enforce users' policies significantly raises the bar for
malicious applications that seek to violate those policies.  However,
like nearly all previous IFC systems~\cite{denning77:_certif,
  myers:jif, efstathopoulos:asbestos, krohn07:_infor_os,
  cheng12:aeolus}, our current implementation does not protect against
malicious attacks outside the scope of the enforcement mechanism,
including timing, termination and probabilistic channels, as well as
physical attacks on trusted components. A malicious application might
be able to export individual bits of information via manipulating
request timing or cache usage, or causing a program to terminate. Such
attacks not only require carefully crafted malicious applications, but
also can only practically exfiltrate small amounts of data -- e.g.,
multiple weeks to extract a credit card
number~\cite{askarov08:_termin_insen_nonin_leaks_more} -- making them
more likely to be detected.


==> background.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-

Today, mobile apps bear the burden of enforcing user policies.  In
this section, we explore why and existing solutions

\subsection{Existing Solutions}
Sharing applications like Facebook offer users simple privacy
policies.  For example, Facebook lets users make posted photos
available to friends, friends of friends, or everyone.  Unfortunately,
even these simple policies are extremely for applications to enforce
because the app must perform access control checks every time the
photo might be displayed to another user. Facebook infamously released
a private photo of founder Mark Zuckerburg holding a dead chicken
because the app did not correctly enforce access control policies for
photos in a poll to
users~\cite{soze11:_mark_zucker_privat_photos_leaked}.

IFC language systems like Jif and others can help programmers track
down these leaks.  However, existing IFC systems are difficult to use,
require programmers to learn a complex IFC model or present some other
barrier to adoption.

Enforcing user policies on untrusted applications is a stronger
solution.  It relieves programmers of the responsibility to implement
correct access control and reduces the trusted code base.  For exactly
this reason, modern mobile OSes enforce access policies on apps for a
set of resources (e.g., those listed in the iOS Privacy Preference or
the Android manifest).

Mobile OSes can effectively enforce policies on mobile devices by
isolating apps or using tools like TaintDroid to ensure apps do not
leak data.  However, sharing apps must move data off of a user's
device in order to share, so the mobile OS has no control over what
Facebook will do once it moves user data off of the phone. 

Distributed solutions that encompass app back-ends have been
proposed. For example $\pi$box isolates each user's private data by
confining it to a sandbox environment that spans both mobile and cloud
nodes. Isolating users in sandboxes makes it easy to enforce privacy
but limits the ways in which users can share data to a restrictive
interface between sandboxes.

IFC operating systems and platforms let users place restrictions on
untrusted applications, but they do not directly support user
policies.  Worse, they require users to understand programming
concepts (e.g., persistent storage vs caching) and anticipate
application behavior (e.g., will the application need access to
persistent storage to work) to correctly set IFC labels.


\paragraph{Information flow control (IFC).}
\agate builds on many of the ideas introduced in previous IFC
systems. However, these systems did not make transparency their goal.
Instead, they were generally proposed as tools to help programmers
build secure applications~\cite{myers:jif, liu:fabric, cheng12:aeolus,
roy09:laminar, yip:data_flow, giffin:hails, schultz13:_ifdb}, IFC
platforms~\cite{giffin:hails} and browser
extensions~\cite{stefan14:cowl}, or to let users place restrictions on
untrusted parts of applications~\cite{efstathopoulos:asbestos,
zeldovich:histar, krohn07:_infor_os} and different untrusted
applications on one device~\cite{nadkarni16:_pract_difc_android}.  In
contrast, \agate uses IFC to a different end: automatically enforce
application users' sharing policies on their data. Towards this end,
it introduces several new design aspects to close the semantic gap
between the application and IFC system.

Agate is most related to TaintDroid, a taint-tracking system for the
Android OS.  However, TaintDroid is a tool for programmers to find
leaks of tainted data, not an IFC privacy-enforcement system.  Thus,
Taintdroid, does not implement full IFC policies but only tracks a
single bit of taint, and it has no enforcement mechanism to prevent
leakage of data.  Further, it is not a distributed platform, so it is
limited to a single mobile device, and is not able to enforce user
policies end-to-end.  Finally, TaintDroid makes different design
decisions as it does not strive to minimize intrusiveness like Agate
but seeks to prevent data leakage.

Like \agate, Laminar~\cite{roy09:laminar} also integrates an operating
system with a language runtime, one of the requirements for
transparent IFC, but to achieve a different goal: to provide a better
programming model which unifies language and OS abstractions. While
Laminar makes the dynamic fine-grained tracking mechanism practical by
having programmers specify lexically scoped security regions, \agate
limits the tracking to mobile OS-protected resources, which are
usually large and few.

% A similar vision for an IFC-based \ppp was proposed in
% W5~\cite{krohn07:_world_wide_web_without_walls} but, to our knowledge,
% was never realized.

% Weir enforces sharing policies
% similar to Agate; however, it only enforces policies between
% applications on a single device.

% Hails~\cite{giffin:hails} is an
% IFC-based framework for programmers to build secure MVC web
% platforms. In this sense, \agate is similar in spirit to platforms
% built in Hails, like GitStar, but \agate limits itself to OS-protected
% resources to achieve transparency, while GitStar defines
% platform-specific resources using Hails abstractions -- a goal similar
% to COWL~\cite{stefan14:cowl}, which integrates IFC with the design of
% existing web browsers. % As a consequence, \agate can support existing
% mobile OS apps. In addition, \agate allows apps to suggest their own
% policies, inspected by the user, while Hails
% % uses a form of mandatory access
% % control (MAC) to
% imposes the platform policies on all of its
% apps. % RIFLE~\cite{vachharajani04:rifle} seeks to protect user privacy
% % via {\em custom low-l
%evel processor hardware} for flow tracking,
% including special CPU instructions and registers. In contrast, \agate
% enforces end-to-end privacy with a distributed software system for
% mobile-cloud apps on commodity hardware.

% IFC enforcement mechanisms vary in multiple dimensions: they can be
% language- or OS-based; they can track information flows at
% granularities ranging from individual variables to entire processes
% and files; and they can enforce restrictions either statically at
% compile-time or dynamically at run-time. One major category of IFC
% systems, including Jif~\cite{myers:dlm, myers:jif} and
% Fabric~\cite{liu:fabric}, uses statically checked, language-based
% fine-grained information flow that requires programmers to label
% individual variables. A second category, dynamic OS-based IFC systems,
% like Asbestos and its successors~\cite{efstathopoulos:asbestos,
%   zeldovich:histar, krohn07:_infor_os}, uses coarse-grained
% information flow tracking that requires the user to label tag
% application processes based on which OS resources (e.g., files and
% sockets) they access. % Once an entire process is tainted, external
% % communication is allowed only when a trusted \emph{declassification}
% % component removes the tag. This application-specific component is
% % allowed to remove IFC restrictions, so it must be written by a trusted
% % developer (or administrator) familiar with an application's
% % structure.
% \agate takes a third approach: dynamic fine-grained information flow
% control, similar to Laminar~\cite{roy09:laminar}. While Laminar makes
% this approach practical by limiting the flow tracking to
% programmer-defined security regions, \agate limits the flow tracking
% to OS-protected resources.

% %%% Local
%Variables: 
%%% mode: latex
%%% TeX-master: "paper"
%%% End: 


==> compliance.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-


We envision several ways for cloud services to become \safe.  First,
Agate provides a \emph{distributed cloud runtime}, called Magma, which
enforces the \safe guarantee on unmodified applications.  Therefore,
applications backends that run in Magma are \safe by construction.
Application providers can verify that their application back-end is
\safe using a TPM to attest that they are running a verified systems
stack including Magma.

Next, we provide a proxy, called Geode, for untrusted cloud services
that do not manipulate user data (e.g., Dropbox, memcached, Redis).
Geode securely encrypts user data and policies before giving them to
the cloud service and enforces user policies when retrieving the data.

Finally, cloud services that do manipulate data can use existing IFC
systems (e.g., Hails~\cite{giffin:hails}) or computation over
encrypted data (e.g., using Mylar~\cite{popa14:mylar}) to ensure that
\safe policies are enforced.  These systems should provide a proof of
correctness for their mechanism to the \safe authority and attest
their code stack using a TPM.

\safe creates a framework to pass user policies and trust from mobile
devices to cloud services.  This framework makes it uniquely possible
for a mobile OS to securely collect user preferences and then ensure
that they are respected across an entire sharing application by only
entrusting user data to \safe services.



==> ifc3.tex <==
% -*- mode: latex; TeX-PDF-mode:t;  reftex-mode:t; TeX-master: "paper";  -*-

\agate's IFC model is similar to other IFC systems with one key
difference: the \agate OS is able to directly map sharing policies to
IFC labels. As a result, the model described in this section is
\emph{transparent} to both programmers and users, meaning neither
needs to understand IFC to use \agate.

% This is important because we do not have to trust programmers or
% users to correctly use the IFC model to ensure that user policies
% are not violated.

\agate automatically tags data from OS-protected resources with user
policies before handing that data (i.e., os-protected resource) to the
application.  The tagged data is passed to the \agate runtime system,
which then propagates and enforces those tags across the entire
distributed application.  Similar to Jif~\cite{myers:jif} and
others~\cite{cheng12:aeolus,liu:fabric}, \agate's information flow
model is based on \emph{principals} and \emph{labels}. There are three
types of IFC principals in \agate -- users, groups and applications --
which map to the principals in \agate sharing policies. Each principal
has a unique \emph{principal id}. There are two types of labels in
\agate: the mutable \emph{data labels}, which carry the sharing
policy, and the immutable \emph{process labels}, which encode
authorization and help enforce the sharing policies.


\paragraph{Data Labels.}
\agate data labels are tags of the form $l
=\set{\principal{o$_1$,
    o$_2$}
  \to \principal{a$_1$,
    u$_1$,
    u$_2$,
    g$_1$}}$,
where \principal{o$_1$, o$_2$} are the user principal ids of the
owners of the labeled data, $\principal{a$_1$}$ is the principal id of
an application allowed to access the labeled data and
$\principal{u$_1$}$, $\principal{u$_2$}$, $\principal{g$_1$}$ are
users and groups allowed to view the labeled data. We will refer to
the set $\{$\principal{a$_1$, u$_1$, u$_2$}, $\forall$ user principal
id $u \in$ \principal{g$_1$}$\}$ as $readers(l)$. \agate attaches an
initial data label to any data read from an OS-protected resource; for
example, when the fitness tracker accesses the GPS on Alice's phone,
\agate labels the returned result with
$\set{\principal{Alice} \to \principal{FitApp, Alice,
    Betty}}$.

% This example label could correspond to Alice's GPS
% sharing policy, where $o1=\id{Alice}$, $a1=\id{FitApp}$,
% $a2=\id{GPSTracker}$, $u1=\id{Betty}$, $u2=\id{Alice}$ and
% $g1=\attrib{Alice}{family}$.  \agate would use this label to taint any
% data from Alice's GPS before handing the data over to the application.
% Because the data comes from an OS-protected resource on Alice's
% phone, the data and any data derived from it belongs to Alice and is
% protected with Alice's \agate sharing policy.

 
%$\set{\id{Alice}, \id{FitApp}: \id{Betty}; \id{GPSTracker}: \id{Alice}, \attrib{Alice}{family}}$. $o1$ is
%  \agate labels
% are a direct representation of \agate sharing policies, which \agate
% automatically applies to OS-protected resources.


\paragraph{Process Labels.}
% \agate process principals
Each \agate application process is labeled with an application
principal (e.g., $\{\principal{a}_1\}$) and, if the process runs on a
mobile device, a user principal (e.g.,
$\{\principal{a}_1, \principal{u}_1\}$).  \agate requires these two to
enforce the two halves of its sharing policies that define
\emph{which} application can access the user's sensitive data and to
\emph{whom} the application can give that data.  The application
principal identifies the application code running in the process,
ensuring that data does not leak to an untrusted app.  For example, if
Alice gives Betty access to her GPS location through her fitness app,
she does not necessarily trust other applications not to leak her
location to Bob (for example, because they use cloud services that
Alice does not trust).  The user principal identifies the owner of the
device where the process runs.
% We give all processes on a mobile device the authority of the
% logged-in user because \agate's trust model assumes that users only
% log in to devices that they trust.

% \agate processes running in the cloud have a root user id,
% meaning that applications can always send data to
% processes of the same application running in the cloud; however, they
% cannot export sensitive data to other user devices unless allowed by
% the sharing policies.

% We trust the
% platform provider to secure their servers against physical attacks and
% to run a verified version of the \agate server.

% Thus, users should only log in to mobile devices that they possess and
% trust (e.g., users should not log in to iPads on display at the Apple
% store).  \agate does not protect the device's OSprotected resources if
% the \agate server has been tampered with or if there is a physical
% attacks on the device itself (e.g., reading data directly from the
% memory bus).

%Unlike processes in coarse-grained dynamic IFC
%systems~\cite{efstathopoulos:asbestos, zeldovich:histar,
%  giffin:hails}, \agate processes do not have information flow labels,
%thus they do not acquire taint as the app runs.
%We describe \agate's fine-grained IFC below.


\paragraph{Information Flow Rules.}

To enforce user sharing policies, \agate must guarantee the following
security property:
\begin{itemize}
\item[] \emph{Data from an OS-protected resource labeled with a
    non-empty initial data label $l_1$ may reach a process labeled
    with label $l_2$ only if $l_2 \subseteq readers(l_1)$}.
\end{itemize}
It does so by applying the following two data and policy propagation
rules:
%\begin{itemize}
\squishlist
\item[] \textbf{Intra-process propagation.} Inside a process, data is
  allowed to flow freely (i.e., no flow control checks are performed)
  but data labels may change. Any data \emph{derived}
%\footnote{As we explain in the next section, 
%  can be derived either through explicit or implicit information flows.}
  from one or more labeled data sources is labeled with a label which
  reflects all the sharing policies involved. For example, if the
  application combines two pieces of sensitive data, their labels are
  \emph{merged} into the resulting label $l$, where the owners are the
  union of the two sets of owners and where $readers(l)$ is the
  intersection of the two sets of readers. That is, given two pieces
  of data with labels $l_1 = \set{\principal{o$_1$} \to readers(l_1)}$
  and $l_2 = \set{\principal{o$_2$} \to readers(l_2)}$, the resulting
  label of any derived data is $\set{\principal{o$_1$,
      o$_2$} \to readers(l_1) \cap readers(l_2)}$.
%\item[]
\item[] \textbf{Inter-process propagation.} Data labeled with the
  current data label $l_1$ is allowed to flow to a process labeled
  with label $l_2$ only if $l_2 \subseteq readers(l_1)$. If the data
  is allowed to flow to the new process, it maintains its label,
  $l_1$, until an intra-process propagation rule is applied.
%\end{itemize}
\squishend

\paragraph{Restricted Resource Declassification.}
\label{sec:restricted_resources}
\agate does not allow untrusted application code to perform
declassification. Instead, \agate includes a set of \emph{restricted
  resources} that inherently provide a less-sensitive view of data
from OS-protected resources, often using data from the mobile OS
(e.g., returning which city a GPS location is in).  When the
application accesses the restricted resource, \agate removes the
original labels on the data object, transforms the data object into
the less-sensitive view, and then attaches new labels corresponding to
the restricted resource sharing policy.  For example, Alice may want
her fitness app to notify Betty when she is in her neighborhood, but
not give Betty her precise location.  While Alice's fitness app can
access her phone's GPS, it would have to transform her location into
the neighborhood before releasing the data to Betty.  Based on Alice's
policy, \agate would add Betty's principal id to the label, thus
enabling Betty to receive notifications without learning Alice's exact
location. Another restricted resource could provide a
busy/available version of the user's calendar.


% IFC systems typically include a \emph{declassification} mechanism
% that allows trusted code to override information flow restrictions by
% removing the label from data.  Although \agate's fine-grained IFC
% mechanism limits its need for declassification, it is sometimes useful
% to declassify a protected resource to support an application function.
% Whereas previous systems let programs with appropriate authority
% arbitrarily declassify resources, \agate does not trust application
% programmers.  As a result, it does not trust \emph{any} application
% code to perform declassification and entirely relies on the trusted
% \agate platform.

% Our key insight is that apps today already rely on the platform to
% provide \emph{transformations} of OS-protected resources (e.g.,
% turning a GPS location into a neighborhood or determining if a
% calendar slot is free). These transformations use data that only the
% OS has (e.g., the neighborhoods in a city) but also inherently
% \emph{degrade} sensitive data before it is shared.

% Thus, rather than allowing applications to invoke arbitrary
% declassification code, \agate provides a set of \emph{restricted
%   resources}, similar to Android's fine vs. coarse GPS location, and
% an interface for applications to request them. When such a request
% occurs, \agate contacts the owner (e.g., Alice) for permission to add
% the policy for the restricted resource. 
% With permission from the
% user,

% Enforcing labels
% \agate servers enforce policies at process boundaries. To check a
% policy, \agate checks the principals listed in the label against the
% principal label on the destination process. The application principals
% must match in the label and for the destination process. Then \agate
% takes the intersection of the user label on the destination process
% and the label on the data. For each group principal in the label, the
% \agate server checks to see if the user principal for the destination
% process is in the group. To find group membership, the \agate server
% contacts the user management service. To avoid the remote access to
% the UMS, \agate servers cache group membership information with a
% lease.


% \paragraph{Limitations}
% \agate's IFC mechanism has several limitations. Since the mechanism
% does not track implicit flows, \agate does not track application data
% derived from sensitive user data. Further, \agate cannot track
% application data derived from user actions (e.g., number of
% Tweets). Since these are applicationinternal concepts, it is
% difficult to imagine users setting policies for them, so we chose to
% limit our tracking mechanism to only data generated by OSprotected
% resources. This choice reduces the overhead of the IFC mechanism and
% the complexity of policies. We believe that limiting our protection
% mechanism only to direct leaks of usergenerated data to be a good
% trade-off of usability and complexity.


==> impl.tex <==
% -*- mode: latex; TeX-PDF-mode:t;  reftex-mode:t; TeX-master: "paper";  -*-

We implemented a prototype that supports distributed Java
applications.  We chose the combination of the Android mobile OS and
the Dalvik language runtime to prototype \agate's co-designed mobile
IFC OS and runtime.  \agate-modified Dalvik VMs run on both Android
devices and x86 servers, but not the \agate mobile OS, so applications
running on x86 servers can pass already tagged data but cannot access
to OS-protected resources.

\subsection{Magma Prototype}

Magma requires way to track both explicit and implicit flows,
represent \agate IFC labels as tags and enforce sharing policies with
IFC checks.  Magma's explicit flow tracking mechanism builds on
TaintDroid~\cite{enck10:taintdroid} for Android 4.3\_r1.  Because
TaintDroid is a simple trait-tracking system and not a full IFC
system, Magma extends its mechanisms significantly.  While TaintDroid
implements very basic taint tracking, e.g., it tracks binary taints
for only 32 sources, Magma uses more complex IFC labels and rules and
performs enforcement checks.

TaintDroid also has no implicit flow tracking. Magma uses a static
analysis tool to insert annotations into Android dex files, then
dynamically propagates labels at runtime. Magma's static analysis tool
was implemented using the Soot framework for Java/Android
apps~\cite{soot}, and consists of 5,400 lines of Java code to perform
class hierarchy analysis, global method call flow analysis, control
flow analysis within methods, side effect analysis inside
conditionals, and insertion of taint tracking code for implicit flows.

% Because Magma using Agate's complex sharing policy labels as tags, 
% The \agate distributed runtime system implements IFC tags as pointers
% to C structures that encode the set of taint labels.  When the runtime
% system receives a new data object from an OS-protected resource, it
% initializes this structure with the user's sharing policy for that
% resource encoded as an IFC label.  The runtime propagates this tag to
% any derived data and modifies it when joining labels. \agate's merge
% function is much more complex than the TaintDroid function on which it
% is based.  TaintDroid uses a simple binary \textsc{or}, while merging
% two tags in \agate requires joining two sets of policies, as described
% in Section~\ref{sec:ifc-model}.  Thus, to reduce runtime overhead, we
% do not intersect the accumulated labels until needed for enforcement
% checks.

% To implement IFC checks, we modified the Android libcore library that
% applications use to access OS functionality.  Our primary task was to
% ensure that data did not violate flow restrictions; e.g., we added
% policy checks to any syscalls (such as \texttt{sendto}) that send data
% to other processes, ensuring that communications do not bypass \agate
% policy checks.  The policy propagation and enforcement required for
% flow control consists of approximately 5800 lines of code.  In
% addition, we modifed 2000 lines of code in Android and TaintDroid to
% support Agate's needs.  New code and modifications are a combination
% of C and Java.

Agate inherits several limitations from TaintDroid. First, data flows
are not tracked through native code. Instead, a conservative heuristic
is used which sets the taint of the result to be a combination of the
taints of the arguments. Second, TaintDroid makes some optimizations
which could lead to over-tainting, such as using a single taint for an
entire array. A newer taint tracking mechanism for JVMs,
Phosphor~\cite{bell14:phosphor}, eliminates some of these issues.

% \subsection{Agate Mobile OS Prototype}
% %Syscall API
% %Sharing Suggestions
% %Declassification Filters

% % \agate users need a secure way to set and review sharing policies on
% % OS-protected resources.

% Android apps access OS-protected resources either through trusted
% applications built into the Android framework (e.g., Calendar,
% Gallery) or directly through system calls (e.g., to access GPS).  The
% current prototype interposes only on calls to the built-in camera and
% GPS resources (i.e., the \texttt{takePhoto()} and
% \texttt{getLastKnownLocation()} system calls); in a full
% implementation, similar modifications would be required for other
% OS-protected resources.

% Our secure UI prototype differs slightly from the design described in
% Sec.~\ref{sec:secureui}.  First, we split the interface for managing
% sharing policies. The Android Manifest already provides users with a
% secure way to set access control policies, so the \agate UI only
% provides settings for flow control. Second, due to current prototype
% limitations, our interface for managing flow control consists of
% dialog boxes drawn in the context of the current application rather
% than in a separate, trusted application.  A more secure prototype
% would show the policy interface in a separate application, as
% demonstrated in prior work~\cite{roesner13:layercake}.

% \paragraph{User Management Service.}
% We implemented a simple UMS using a centralized database to store the
% users and their associated groups. Our prototype provides user
% authentication and group management, and maps usernames and groupnames
% to principal ids used for IFC labels and sharing policies.











==> motivation.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-

Information flow control (IFC) offers a solution for enforcing user
privacy in sharing applications; unfortunately, existing IFC systems
are not designed to support existing sharing policies, making them
difficult for both users and programmers to adopt.  In this section,
we review sharing policies commonly used in today's social
applications and existing IFC systems. Finally, we describe Agate's
challenges in bridging the semantic gap between the two.

\subsection{Sharing Policies}
Today's mobile app users can control access to their sensitive data
with two types of policies.  First, mobile operating systems offer
privacy controls (e.g., Android Manifest, iOS Privacy Settings), which
let users restrict application access to sensitive data sources (e.g.,
GPS, contact list). For example, Alice might give a running app,
\textsc{RunWithMe} (similar to MapMyRun~\cite{mapmy}), access to her
GPS location.  Second, mobile applications offer privacy settings,
which let users control the sensitive data shared with other users.
As an example, Alice might allow \textsc{RunWithMe} to share her GPS
location with her running partner Betty.

This division between policies today is less than ideal.  While Alice
trusts her mobile OS to limit access to her GPS sensor, she may not
trust \textsc{RunWithMe} to preserve her privacy and limit her GPS
location to Betty.  Likewise, while we might expect mobile OS
developers to correctly implement privacy policies, expecting
applications developers to do the same is more difficult.

Unfortunately, there exist no general-purpose systems today that can
enforce both types of policies.  Applications run across many mobile
devices and cloud servers where mobile operating systems do not
extend.  There has been research into distributed platforms that
isolate users (e.g.,
$\pi$box~\cite{sangmin:pibox,lee14:_clean_approac_byoa} or encrypt
user data (e.g., Mylar~\cite{popa14:mylar}) but these systems only
support limited sharing features.

\subsection{IFC Systems}
IFC systems were originally designed to help programmers prevent
information leaks in their applications.  To use these systems,
programmers label sensitive application data and components, and then
the system tracks and controls the flow of labeled data.  For example,
language-based IFC systems (e.g., Jif~\cite{myers:jif},
Fabric~\cite{liu:fabric}, Jeeves~) need programmers to label
application variables or define IFC policies. OS-based IFC systems
(e.g., Asbestos~\cite{efstathopoulos:asbestos},
Flume~\cite{krohn07:_infor_os}, HiStar~\cite{zeldovich:histar})
require a system administrator or advanced user to separate and label
application components based on their access rights.  Labeling
variables or components incorrectly can lead to data leaks or
overtainting, which then requires complex declassification to fix.
Distributed IFC web frameworks (e.g., Hails~\cite{giffin:hails},
COWL~\cite{stefan14:cowl}, Aeolus~\cite{cheng12:aeolus}, Stoplight 

Existing IFC systems have a semantic gap between user sharing
policies, which use user-friendly concepts like mobile resources
(e.g., GPS) or users (e.g., Betty), and IFC labels and policies, which
refer to programming concepts like variables, persistent storage,
caching.  This gap leaves the user with two choices: (1) understand
these programming concepts enough to correctly set their policies, or
(2) trust someone else to correctly implement their policy in IFC
labels for every application that they use (e.g., a programmer or a
third party like the EFF).  Agate explores a third option by bridging
the semantic gap between existing sharing policies and IFC. 

\subsection{Bridging the Gap}


Agate supports existing sharing policies through a new IFC mechanism,
which we call \emph{transparent IFC}.  The goal of transparent IFC is
to enforce existing user policies without requiring the user or the
programmer (or any third party) to interact with the IFC mechanism.
Achieving transparent IFC requires several

  \begin{table}[t]
%\vspace{-.1in}
  \centering
  \caption{Examples of mobile OS-protected resources and applications
    that use them to share data with other users.}
  %\vspace{.1in}
  {\small
    \def\arraystretch{1.0}
    \def\cellset{\def\arraystretch{1}}
    \def\theadfont{\bfseries\footnotesize}
    \def\theadalign{ll}
    \def\theadset{\def\arraystretch{1.3}}%
    \def\cellalign{l}
    \begin{tabular}{@{}ll@{}}
      \toprule
      \thead{OS Resource}
      &\thead{Example Applications}\\
      \midrule
      Camera 
      & Twitter~\cite{twitt}, Snapchat~\cite{snapc}, WellsFargo~\cite{wells} \\
      Contacts 
      & Foursquare~\cite{fours}, WordsWithFriends~\cite{words_with_frien}\\
      GPS location & Uber~\cite{ub}, Zillow~\cite{zillow},  MapMyRun~\cite{mapmy} \\
      Sensors & Fitbit~\cite{fitbit}, Pedometer~\cite{pedom}, Nike$+$~\cite{nike_runnin_app} \\
      Microphone & WeChat~\cite{wechat}, Skype~\cite{skype}, Google Trans.~\cite{googl_trans} \\
      Calendar& Pick~\cite{pick}, Hub~\cite{hub}, Genee~\cite{genee}, 2Do~\cite{do}\\
      Credit cards & Ticketmaster~\cite{ticket}, Amazon~\cite{amazon_shopp}, Saks~\cite{saks} \\
      \bottomrule
  \end{tabular}}
  \label{tab:resources}
\end{table}

% A way to identify data to be labeled - we limit tracked data to
% a way to identify and label processes
% a way to avoid overtainting and declassification


==> motivation2.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-


Important trends in the mobile environment make \agate's transparent
IFC possible.  In this section, we discuss how each trend motivates a
drastic departure in \agate's design from previous IFC systems and
moves \agate closer to its goal of achieving transparent IFC.
Table~\ref{tab:ifc_systems} compares the design of existing IFC
systems to \agate and evaluates them on their transparency.

\subsection{Trend 1: Mobile OS and Language Integration}

Mobile apps are implemented largely in one language (i.e., Java or
Swift), execute in a single user-level language runtime (i.e., Dalvik
JVM or Objective-C runtime) and run on a specialized OS (i.e., Android
or iOS).  This property allows \agate to tightly integrate the OS and
language runtime in a way that is impossible for past IFC systems.
For example, IFC language systems, like Jif~\cite{myers:jif} and
Fabric~\cite{liu:fabric, arden:mobile_fabric}, cannot require the
operating system to manage complex IFC policies and label sensitive
data, so programmers must manually label application variables.
Likewise, operating systems like HiStar~\cite{zeldovich:histar} cannot
make assumptions about the application programming language and its
runtime, so they must rely on coarse-grained tracking that works for
all languages, including low-level languages like C. For example,
HiStar users must partition their applications into components using
six types of kernel objects (e.g., process, gate, memory segment);
then, each kernel object must be labeled with a set of categories,
each having one of six security levels. Done incorrectly, application
components will rapidly acquire taint, making it difficult for the
application to do anything useful without complicated declassification.

\begin{table}[t]
%\vspace{-.1in}
  \centering
  \caption{Examples of mobile OS-protected resources and applications
    that use them to share data with other users.}
  %\vspace{.1in}
  {\small
    \def\arraystretch{1.0}
    \def\cellset{\def\arraystretch{1}}
    \def\theadfont{\bfseries\footnotesize}
    \def\theadalign{ll}
    \def\theadset{\def\arraystretch{1.3}}%
    \def\cellalign{l}
    \begin{tabular}{@{}ll@{}}
      \toprule
      \thead{OS Resource}
      &\thead{Example Applications}\\
      \midrule
      Camera 
      & Twitter~\cite{twitt}, Snapchat~\cite{snapc}, WellsFargo~\cite{wells} \\
      Contacts 
      & Foursquare~\cite{fours}, WordsWithFriends~\cite{words_with_frien}\\
      GPS location & Uber~\cite{ub}, Zillow~\cite{zillow},  MapMyRun~\cite{mapmy} \\
      Sensors & Fitbit~\cite{fitbit}, Pedometer~\cite{pedom}, Nike$+$~\cite{nike_runnin_app} \\
      Microphone & WeChat~\cite{wechat}, Skype~\cite{skype}, Google Trans.~\cite{googl_trans} \\
      Calendar& Pick~\cite{pick}, Hub~\cite{hub}, Genee~\cite{genee}, 2Do~\cite{do}\\
      Credit cards & Ticketmaster~\cite{ticket}, Amazon~\cite{amazon_shopp}, Saks~\cite{saks} \\
      \bottomrule
  \end{tabular}}
  \label{tab:resources}
\end{table}

\begin{table*}[t!]
%\vspace{-.1in}
  \centering
  \caption{Summary of existing IFC systems. We evaluate each system on
    its transparency (i.e., the burden on programmers and users).  We
    consider code modifications to be a higher burden than supporting
    untrusted applications.  Each system's transparency depends on the
    amount of management done by the OS instead of the app or user. Agate leverages trends in the mobile environment to move all management into the OS, making it the only highly transparent IFC system.}

    \vspace{.1in} {\footnotesize \def\arraystretch{1.0}
      \def\cellset{\def\arraystretch{1}}
      \def\theadfont{\bfseries\footnotesize} \def\theadalign{ll}
      \def\theadset{\def\arraystretch{1.3}}%
      \def\cellalign{l}
    \begin{tabular}{@{}llllllll@{}}
      \toprule
      \thead{System Type}
      &\thead{System Name}
      &\thead{Transparency}
      &\thead{Source of\\Protected Data}
      &\thead{User\\Management}
      &\thead{Policy\\Management}
      &\thead{Labeller}
      &\thead{Declassifier}
      \\
      \midrule
      \multirow{2}{*}{\makecell{Integrated\\(Language \& OS)}}
      & Agate
      & High
      & OS
      & OS
      & OS
      & OS
      & OS
      \\
      & Laminar~\cite{roy09:laminar}
      & Medium
      & OS/App
      & App
      & App
      & Programmer
      & Programmer \\
      \midrule
      \multirow{4}{*}{Operating System}
      & Asbestos~\cite{efstathopoulos:asbestos}
      & Medium
      & OS
      & App
      & User
      & User
      & User\\
      & Flume~\cite{krohn07:_infor_os}
      & Medium
      & OS
      & App
      & User
      & User
      & User \\
      & HiStar~\cite{zeldovich:histar}
      & Medium
      & OS
      & OS/App
      & User
      & User
      & User \\
      & DStar~\cite{zeldovich:dstar}
      & Medium
      & OS
      & App
      & User
      & User
      & User\\
      \midrule
      \multirow{2}{*}{\makecell{Language\\(Dynamic)}}
      & Aeolus~\cite{cheng12:aeolus}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer\\
      & Resin~\cite{yip:data_flow}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer\\
      \midrule
      \makecell{Language\\(Dynamic \& Static)}
      & COWL~\cite{stefan14:cowl}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer\\
      \midrule
      \multirow{3}{*}{\makecell{Language\\(Static)}}
      & Fabric~\cite{liu:fabric, arden:mobile_fabric}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer\\
      & Jif~\cite{myers:jif}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer \\
      & Sif~\cite{chong07:sif}
      & Low
      & App
      & App
      & App
      & Programmer
      & Programmer\\
      \bottomrule
  \end{tabular}}
  \label{tab:ifc_systems}
\end{table*}

Tight integration between the runtime and OS gives \agate the benefits of
both IFC language systems and operating systems.  Like IFC operating
systems, \agate is able to run untrusted applications because it
manages policies and labels sensitive data automatically. Like IFC
language runtime systems, \agate is able to perform fine-grained,
dynamic explicit and implicit flow tracking to avoid over-tainting and
complex declassification.  By passing information between the OS and
language runtime, \agate eliminates the need for programmers or users
to bridge the semantic gap between the application and IFC model,
bringing it one step closer to transparent IFC.




\subsection{Trend 2: Diverse OS-Protected Resources}
% rather than coarse grained tracking, we perform fine-grained
% tracking on few objects


To make dynamic, fine-grained tracking practical, IFC systems limit
their taint-tracking to a subset of the application. For example,
Resin~\cite{yip:data_flow} limits tracking to assertions, and
Laminar~\cite{roy09:laminar} only tracks flows in particular regions
of code.  However, both solutions require programmers to choose which
data to track, so they cannot be used for \agate.

Instead, \agate limits its taint tracking to OS sources. Unlike
conventional operating systems, mobile OSes manage an increasingly
varied set of sensitive data sources with rich semantics and privacy
policies.  To differentiate from traditional OS sources (e.g., files,
sockets), we call these {\em mobile OS-protected resources}.  These
resources can be divided into two categories: \emph{hardware
  resources} (e.g., GPS, camera), which the mobile OS protects along
with securely managing the data derived from them (e.g., iOS Camera
and Photos app), and \emph{software resources}, which securely collect
personal data, like the user's calendar, contacts and credit
cards. Table~\ref{tab:resources} gives examples of many OS-protected
resources and applications that share their data.

Data objects from OS-protected resources are typically large (e.g.,
photos, voice message, calendar events) and, at the same time, make up only a small
amount of the overall data in an application.  Further, they are not
frequently combined with other application data (e.g., a GPS or credit
card number is an immutable object) or used for control flow (e.g.,
photos are typically not used inside  the conditions of \emph{if} statements), reducing the possibility of over-tainting.

\agate does not eliminate declassification.  Instead of
general-purpose declassification, which requires programmers or users
to manually remove IFC labels, \agate provides \emph{OS-restricted
  resources} (Sec.~\ref{sec:restricted_resources}), a set of
extensible and trusted APIs which operate on OS-protected resources.
OS-restricted resources use the semantics of OS-protected resources to
automatically reduce taint.  Altogether, limiting privacy enforcement
to mobile OS-protected resources with their rich set of semantics
brings \agate another step closer to transparent IFC.


\subsection{Trend 3: Centralized User Management}
A key remaining barrier to transparent IFC is user management.  In
particular, any IFC system that does not understand principals and
policies requires a programmer or user to translate application
policies to IFC labels.  Fortunately, the mobile environment lets
\agate make two important simplifying assumptions: (1) every mobile
app on a device belongs to a single user (e.g., Android apps support a single user
at a time), and (2) users authenticate through a centralized user
management service (e.g., with their AppleID~\cite{apple_id}) before
accessing apps.

% Unlike
% general-purpose operating systems, mobile OSes are designed to support
% a single user with a single account (e.g., AppleID~\cite{apple_id}).
% In addition, modern mobile apps typically do not implement user
% management themselves, instead relying on a variety of global user
% identification and authentication services (e.g., Facebook Login [23]
% or Google Identity Platform [32]).  As a result, we can assume that
% \agate can use these services to verify principals and associate
% devices with those principals.

With these assumptions, \agate gives all processes on a device the
permissions of the authenticating user and attributes all data
collected from OS-protected resources to that user.  Further, \agate
leverages these user principals to define \emph{sharing policies},
which specify the other users that the application can allow to access
a user's sensitive data.  Because these user principals are valid
across devices and understandable to the application and user (e.g.,
they represent the user's friends), applications use them to propose
custom policies for users to accept or reject.  Once set, \agate can
translate these policies into meaningful labels on data from
OS-protected resources, allowing \agate to enforce sharing policies
transparently with IFC.

%\begin{table*}[t!]
%%\vspace{-.1in}
%  \centering
%  %\vspace{.1in}
%  {\small
%    \def\arraystretch{1.0}
%    \def\cellset{\def\arraystretch{1}}
%    \def\theadfont{\bfseries\footnotesize}
%    \def\theadalign{ll}
%    \def\theadset{\def\arraystretch{1.3}}%
%    \def\cellalign{l}
%    \begin{tabular}{@{}lllllll@{}}
%      \toprule
%      &\thead{Untrusted apps?} 
%      &\thead{Who sets labels?}
%      &\thead{Labeled resources}
%      &\thead{Principals}
%      &\thead{Enforcement mechanism}
%      \\
%      \midrule
%      \textbf{Agate} & \textbf{Yes} & \textbf{Mobile
%OS users} & \textbf{Mobile OS resources} & \textbf{Mobile OS} & %\textbf{dynamic, fine-grained} \\
%      \hline
%      \makecell[l]{Asbestos~\cite{efstathopoulos:asbestos} \\
%Flume~\cite{krohn07:_infor_os} \\ HiStar~\cite{zeldovich:histar} \\ %DStar~\cite{zeldovich:dstar}} &
%Yes & User/App-defined & \makecell[l]{OS processes, files, \\ %sockets, mem pages, etc.} & Users & dynamic,
%coarse-grained \\
%      \hline
%      \makecell[l]{Aeolus~\cite{cheng12:aeolus} \\ %COWL~\cite{stefan14:cowl}} &
%No & App-defined & \makecell[l] {App data objects, \\ threads/tasks} %&
%Programmers & dynamic, coarse-grained \\
%      \hline
%      Jif~\cite{myers:jif} & No & App-defined & App variables, %functions & Programmers &
%static, fine-grained \\
%      \hline
%      Resin~\cite{yip:data_flow} & No & App-defined & App data %objects & Programmers &
%dynamic, fine-grained \\
%      \hline
%      Laminar~\cite{roy09:laminar} & No & App-defined & %\makecell[l]{App data objects, \\ OS resources} & Programmers & %dynamic, fine-grained \\
%      \bottomrule
%  \end{tabular}}
%  \caption{Previous IFC systems allow applications and users to %define and manage the principals (owners of sensitive data) while %\agate's principals are the users of the mobile OS. Like \agate, OS-
%level solutions (second row) support untrusted applications but with %significantly higher burden on the users. Several runtime solutions %allow for less complex labeling schemes (Aeolus, Resin) but they must %trust programmers.}
%  \label{tab:ifc_systems}
%\end{table*}


==> policies2.tex <==
% -*- mode: latex; TeX-PDF-mode:t;  reftex-mode:t; TeX-master: "paper";  -*-

Users control the sharing of OS-protected resources with {\em \agate
  sharing policies}. These policies integrate both access and flow
control by specifying: (1) which resources an application can access,
and (2) how the application can export data derived from that
resource.  For example, in Figure~\ref{fig:arch}, \agate permits
Alice's photo to be passed to an application and then to Betty, while
it prevents the photo from being shared with Bob.  This is a
significant improvement to today's mobile OSes (e.g., Android and
iOS), where the former is handled by permissions set using
install-time manifests and runtime prompts, while the latter is
entrusted to applications.

\agate sharing policies are expressed in terms of \emph{users},
\emph{groups}, and \emph{applications}. Each policy maps an
OS-protected resource to an application that is allowed to access it
and the list of users and groups with which the app can share that
data.  For example, Alice can set a policy allowing her fitness app to
access her GPS and to share her GPS-derived data only with Betty. We
use the following notation to denote Alice's sharing policy:
$\resource{GPS} = \tup<\app{FitApp},\set{\principal{Betty}}>$. Note
that this policy only allows Fitapp to share Alice's GPS-derived data
with Betty, not other applications.  Users can also define policies
for their restricted resources. For example, to let another app share
Alice's current neighborhood but not her precise location with Betty,
Alice could define
$\exception{GPS}{Neighborhood} =
\tup<\app{FriendApp},\set{\principal{Betty}}>$.

\agate's policies preserve the existing user experience. Users already
have such policies in mind but typically specify them through
in-application interfaces (e.g., a dialog box in which the user
selects with whom to share a photo).  In contrast, \agate bypasses the
application, securely collects user policies through its mobile OS and
enforces those policies in the platform itself.

While users ultimately set or approve all policies, \agate allows
applications to suggest policies in several ways.  First, applications
can create \agate groups that map to application-specific
concepts. For example, Alice's fitness application could define
$\group{Alice}{Running-Group}$, which lets Alice share her runs with
all of her running partners. Next, \agate provides an API for
applications to propose policies. For example, Alice's fitness app
might offer her the choices
%$\resource{GPS} = \tup<\app{FitApp}, \set{}>$
$\resource{GPS} = \tup<\app{FitApp}, \set{\principal{Alice}}>$ and
$\resource{GPS} = \tup<\app{FitApp}, \set{\principal{Alice},
  \group{Alice}{running-group}}>$
to only share data from the GPS across Alice's devices or with her group.


==> providers.tex <==
% -*- mode: latex; TeX-PDF-mode:t; reftex-mode:t; TeX-master: "paper"; -*-


\begin{figure}[t]
  \centering
  \addfigure{simplified_arch.pdf}
  \caption{User trust model. The shaded area surrounds the components
    the user must trust with her sensitive data.  Currently (a) Alice
    must trust her mobile OS, cloud provider and all of her apps to
    enforce her privacy policy (e.g., do not leak her GPS location to
    Bob). \agate (b) introduces a trusted privacy-preserving platform
    (\ppp) that is responsible for enforcing Alice's policy on her
    applications, eliminating the need for her to trust her
    applications.}
  \label{fig:simplified_arch}
\end{figure}

Today, users set privacy policies on their personal data and trust a
number of entities to enforce them.  For example, Alice wants her
fitness app to share her GPS location with Betty but not Bob.  As
shown in Figure~\ref{fig:simplified_arch}(a), Alice must trust: (1)
her mobile OS to limit access to her GPS, (2) her social fitness app
to only share her location with Betty, and (3) her cloud platform and
Betty's mobile OS to not leak her location to Bob.

While Alice and Betty each use one mobile OS and cloud platform, Alice
may need to give dozens of apps access to her GPS.  For example, she
may want to allow a social meetup app to show her current location to
friends or Twitter to geo-tag her tweets.  Currently, she must trust
all of those apps to respect her privacy policy.  Whether an app is
incomplete, buggy or malicious, the result is the same: only a single
app needs to inadvertently leak Alice's GPS location for Bob to find
her.

For this reason, \agate embraces the concept of a
\emph{privacy-preserving platform} (\ppp) -- a trusted layer whose
only responsibility is enforcing privacy guarantees.  As shown in
Figure~\ref{fig:simplified_arch}(b), the \agate \ppp runs code from
untrusted application developers and prevents them from leaking data
that is prohibited by the user's policy. Now, in addition to the \ppp,
Alice only needs to trust her and Betty's mobile OSes and cloud
platform to be confident that her GPS location will not be leaked to
Bob, a significant improvement from today's model.

Both users and application developers benefit from outsourcing privacy
policy enforcement to a separate \ppp layer. Users can trust that
their privacy policies are upheld even if the application is
untrustworthy or buggy -- an important benefit in a world of millions
of largely anonymous developers and apps.  And developers no longer
have to be security experts, perfectly implementing complex privacy
features to avoid leaks; thus, they benefit from increased trust and
assurance, and can use the \agate \ppp as a ``safety net'' to prevent
unintentional data disclosure.  Given that the \ppp's primary job is
to maintain user privacy guarantees, Alice can be confident her policy
is followed, even if she does not fully trust her application or their
programmers.

We do not explicitly address the question of who should be the \ppp
provider. They could be the same as the mobile OS or cloud platform
provider (i.e., Apple, Google, Microsoft) but do not have to be.  We
note that today's mobile/cloud applications \emph{already} rely on a
variety of platform providers, some of which are already responsible
for security functions, including global user identification and
authentication services (e.g., Facebook Login~\cite{facebook-login} or
Google Identity Platform~\cite{google-sso}), and trusted, curated
central app stores (e.g., Apple's iOS~\cite{apple_app_store} and
Google's~\cite{googl_play} Android app stores). The companies involved
with these services increasingly view protecting the privacy of user
data as a competitive advantage~\cite{macworld14:_why_apple,
  wingfield13:_micros_attac_googl_gmail_privac}, making them plausible
candidates to support a privacy-preserving platform.


==> ums.tex <==
% -*- mode: latex; TeX-PDF-mode:t;  reftex-mode:t; TeX-master: "paper";  -*-

The \safe user service has two primary roles: (1) securely managing
the principles used to express sharing policies, including group
membership management, and (2) verifying user identities for \safe
OSes to authorize the release of data from \safe cloud service
according to \safe policies.  The \safe user service gives every
application, user and group a unique identifier and stores a mapping
between names and ids.  It also stores user passwords, and, for each
group, the group owner and membership.

When a user logs in to a \safe mobile OS like Agate, the OS sends the
request to the \safe user service, which verifies the user identity
(by checking the password). If verified, \safe user service issues the
OS a time-limited certificate for that user authorizing the OS to do
the following on behalf of that user: (1) collect data from the mobile
device, (2) query and set policies for data from the user, (3) modify
the user's group membership and the membership of any groups owned by
the user, and (4) share user data with \safe cloud services or other
OSes according to the sharing policy.  A \safe OS can present this
certificate to \safe cloud services and OSes to prove that it is
running on a device trusted by the user and thus can accept sensitive
data if the \safe policy includes the user.

The \safe user service is not {\safe}-specific; there are many
existing single-sign-on (SSO) services that could be used to implement
the same functionality (e.g., Google Accounts~\cite{googl_accoun},
OpenID~\cite{openid}).  The only requirement is that the service be
able to authenticate users, issue certificates and manage group
membership.  For trust reasons, we assume that \safe user service is
implemented and deployed by an entity separate from the application
provider; otherwise, we would have to trust the application to manage
users, which many fail at~\cite{linked_hack,17:_mohit_kumar}.


